Develop End-to-End Anomaly Detection System

Anomaly detection plays a crucial role in ensuring network robustness. However, implementing intelligent alerting systems becomes a challenge when considering scenarios in which anomalies can be caused by both malicious and non-malicious events, leading to the difficulty of determining anomaly patterns. The lack of labeled data in the computer networking domain further exacerbates this issue, impeding the development of robust models capable of handling real-world scenarios. To address this challenge, in this paper, we propose an end-to-end anomaly detection model development pipeline. This framework makes it possible to consume user feedback and enable continuous user-centric model performance evaluation and optimization. We demonstrate the efficacy of the framework by way of introducing and bench-marking a new forecasting model -- named \emph{Lachesis} -- on a real-world networking problem. Experiments have demonstrated the robustness and effectiveness of the two proposed versions of \emph{Lachesis} compared with other models proposed in the literature. Our findings underscore the potential for improving the performance of data-driven products over their life cycles through a harmonized integration of user feedback and iterative development.

==> tables/balanced_w26_w27_w28.tex <==
\floatstyle{plaintop}
\restylefloat{table}
\begin{table*}[t]
    %\centering
    \caption{Performance metrics of a balanced batch of nodes}
    \label{tab:bactch_balanced}
    
    \begin{adjustbox}{width=2.2\columnwidth, keepaspectratio}
    \begin{tabular}{c|c|c|c|c|c|c}
        \hline
        \makecell{\textbf{Model}} & \makecell{\textbf{MSE}} & \makecell{\textbf{RMSE}} & \makecell{\textbf{MAE}} & \makecell{\textbf{Avg. Daily Alerted} \\ \textbf{Nodes}} &  \makecell{\textbf{Avg. Daily} \\ \textbf{Alerts}} & \makecell{\textbf{Total Alerts}}  \\
        \hline
        \makecell{arima} & 1769.932±196.916 & 42.027±2.335 & 12.423±0.685 & 56.095±5.288 & 110.714±17.693 & 775±123.851 \\
        \makecell{dlm} & 1769.038±612.300 & 41.622±7.418 & 11.907±2.629 & 71.381±6.671 & 158.571±18.548 & 1110±129.835 \\
        \makecell{lachesis\_v0} & \textbf{4.990±0.227}	& \textbf{2.234±0.051}	& \textbf{1.184±0.018} & 85.667±2.144	& 210.238±9.915	& 1471.667±69.407 \\
        \makecell{lachesis\_v1} & 3430.788±904.687 & 58.23±7.756 & 55.176±7.454 & \textbf{15.048±4.908}	& \textbf{33.333±15.369} & \textbf{233.333±107.584} \\
        \makecell{linear} & 1671.404±318.552	& 40.752±4.003	& 13.624±1.260 & 67.714±5.878	& 150.191±21.976	& 1051.333±153.832 \\
        \makecell{phase1} &15305014±6820400 & 3833.331±957.016	& 563.420±95.862 & 21.857±10.933	& 33.524±19.873	& 234.667±139.113 \\
        \makecell{prophet} & 2353.651±886.237	& 47.953±9.014	& 14.039±2.876 & 65.476±6.118	& 135.524±16.993	& 948.667±118.951 \\
        \makecell{quadratic} & 2018.9±93.3	& 44.924±1.044	& 14.43±1.273 & 66.905±7.593	& 140.619±20.991	& 984.333±146.937 \\
        \makecell{sarima} & 4183.916±706.578	& 64.535±5.359 & 16.669±2.290 & 33.714±3.714	& 60.762±5.915	& 425.333±41.405 \\
        \hline
    \end{tabular}
    \end{adjustbox}

    \vspace{10pt}
    
    \begin{adjustbox}{width=1.8\columnwidth, keepaspectratio}
    \begin{tabular}{c|c|c|c|c}
        \hline
        \textbf{Model} & \makecell{\textbf{t\_train (s) / 1k} \\ \textbf{data points}} & \makecell{\textbf{t\_infer (s) / 1k} \\ \textbf{data points}} & \makecell{\textbf{t\_train (s) / 1k} \\ \textbf{nodes}} & \makecell{\textbf{t\_infer (s) / 1k} \\ \textbf{nodes}} \\
        \hline
        \makecell{arima} & 0.378±0.230	& 0.181±0.099	& 317.738±193.736	& 30.523±16.754 \\
        \makecell{dlm} & 0.685±0.21	& 1.18±0.696	& 576.1±176.809	& 199.337±117.699 \\
        \makecell{lachesis\_v0} & 0.149±0.03	& 0.866±0.138	& 7508.336±1511.362	& 8734.203±1394.595 \\
        \makecell{lachesis\_v1} & 0.3995±0.107	& \textbf{0.0005±0.0002}	& 20132.882±5398.693	& 5.1030±1.98\\
        \makecell{linear} & 0.0057±0.0031	& 0.03±0.015	& 4.8±2.567	& 5.065±2.48 \\
        \makecell{phase1} &\textbf{0.0025±0.0010}	& 0.043±0.013	& \textbf{2.063±0.81}	& 7.297±2.126 \\
        \makecell{prophet} & 0.27±0.06	& 0.756±0.229	& 228.916±50.335	& 127.78±38.72 \\
        \makecell{quadratic} & 0.0055±0.0025	&0.0298±0.0092	&4.654±2.08&	\textbf{5.033±1.554} \\
        \makecell{sarima} & 3.669±1.704	& 0.274±0.168	& 3085.996±1433.175	& 46.365±28.392 \\
        \hline
    \end{tabular}
    \end{adjustbox}
    
    \vspace{10pt}

    \begin{adjustbox}{width=1.8\columnwidth, keepaspectratio}
    \begin{tabular}{c|c|c|c|c}
        \hline
        \makecell{\textbf{Model}} & \makecell{\textbf{TP}} & \makecell{\textbf{FP}} & \makecell{\textbf{TN}} & \makecell{\textbf{FN}} \\
        \hline
    \makecell{arima} & 131.333±24.583 & 643.667±99.962 & 19366.667±187.431 & 6602.667±2978.339 \\
    \makecell{dlm} & \textbf{185.667±22.008} & 924.333±109.441 & 18914±337.23 & \textbf{6548.33±2949.41} \\
    \makecell{lachesis\_v0} & 166±8.19 & 1305.667±64.933 & 14297±576.27 & 6568±2961.09 \\
    \makecell{lachesis\_v1} & 109±42.93 & \textbf{124.33±73.078} & 20154.667±240.80 & 6625±3008.168 \\
    \makecell{linear} & 180.333±21.008 & 871±135.193 & 18823.667±296.659 & 6553.667±2970.17 \\
    \makecell{phase1} & 61.333±11.930 & 173.333±135.711 & \textbf{20293.667±204.962} & 6672.667±2959.571 \\
    \makecell{prophet} & 160.667±14.364 & 788±115.5 & 19118.33±287.77 & 6573.33±2952.52 \\
    \makecell{quadratic} & 177.33±23.71 & 807±126.69 & 18951±424.72 & 6556.67±2953.11 \\
    \makecell{sarima} & 97.33±3.79 & 328±37.8 & 19986±267.1 & 6636.67±2969.4 \\
    \hline
\end{tabular}
\end{adjustbox}

\vspace{10pt}

    \begin{adjustbox}{width=2\columnwidth, keepaspectratio}
    \begin{tabular}{c|c|c|c|c|c}
        \hline
        \makecell{\textbf{Model}} & \makecell{\textbf{accuracy}} & \makecell{\textbf{precision}} & \makecell{\textbf{recall}} & \makecell{\textbf{specificity}} 
        & \makecell{\textbf{balanced accuracy}}\\
        \hline
    \makecell{arima} & 0.734±0.078 & 0.169±0.008 & 0.023±0.012 & 0.968±0.005 & 0.495±0.004\\
    \makecell{dlm} & 0.724±0.081 & 0.167±0.007 & 0.0305±0.0110 & 0.953±0.006 & 0.492±0.006\\
    \makecell{lachesis\_v0} & 0.654±0.0901 & 0.113±0.005 & 0.028±0.011 & 0.916±0.004 & 0.472±0.006\\
    \makecell{lachesis\_v1} & \textbf{0.7556±0.0819} & \textbf{0.4786±0.1171} & 0.020±0.014 & \textbf{0.9939±0.0035} & \textbf{0.5070±0.0056}\\
    \makecell{linear} & 0.7245±0.0762 & 0.172±0.011 & \textbf{0.0305±0.0143} & 0.956±0.007 & 0.4931±0.0043\\
    \makecell{phase1} & 0.7535±0.077 & 0.3096±0.1365 & 0.010±0.004 & 0.9916±0.0066 & 0.500±0.001\\
    \makecell{prophet} & 0.729±0.079 & 0.171±0.021 & 0.0264±0.0090 & 0.96±0.006 & 0.493±0.004\\
    \makecell{quadratic} & 0.73±0.08 & 0.18±0.01 & 0.029±0.012 & 0.959±0.007 & 0.494±0.005\\
    \makecell{sarima} & 0.748±0.080 & 0.2297±0.0141 & 0.016±0.007 & 0.984±0.002 & 0.5±0.003\\
    \hline
\end{tabular}
\end{adjustbox}


    
\end{table*}


\begin{comment}
    \begin{adjustbox}{width=2.5\columnwidth, keepaspectratio}
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c}
        \hline
        \makecell{\textbf{Model}} & \makecell{\textbf{TP}} & \makecell{\textbf{FP}} & \makecell{\textbf{TN}} & \makecell{\textbf{FN}} & \makecell{\textbf{accuracy}} & \makecell{\textbf{precision}} & \makecell{\textbf{recall}} & \makecell{\textbf{specificity}} 
        & \makecell{\textbf{balanced accuracy}}\\
        \hline
        \makecell{arima} & 131.333±24.583	&643.667±99.962	&19366.667±187.431	&6602.667±2978.339	&0.734±0.078	&0.169±0.008	&0.023±0.012	&0.968±0.005	&0.495±0.004\\
        \makecell{dlm} & \textbf{185.667±22.008}	& 924.333±109.441	&18914±337.23	&\textbf{6548.33±2949.41}	&0.724±0.081	&0.167±0.007	&0.0305±0.0110	&0.953±0.006 &0.492±0.006  \\
        \makecell{lachesis\_v0} & 166±8.19	&1305.667±64.933	&14297±576.27&	6568±2961.09	&0.654±0.0901	&0.113±0.005	&0.028±0.011	&0.916±0.004	&0.472±0.006\\
        \makecell{lachesis\_v1} & 109±42.93	&\textbf{124.33±73.078} & 20154.667±240.80	&6625±3008.168	&\textbf{0.7556±0.0819}	&\textbf{0.4786±0.1171} &0.020±0.014	&\textbf{0.9939±0.0035}	&\textbf{0.5070±0.0056} \\
        \makecell{linear} & 180.333±21.008&	871±135.193	&18823.667±296.659&	6553.667±2970.17	&0.7245±0.0762	&0.172±0.011	&\textbf{0.0305±0.0143}	&0.956±0.007&	0.4931±0.0043\\
        \makecell{phase1} &61.333±11.930	&173.333±135.711	&\textbf{20293.667±204.962}	&6672.667±2959.571	&0.7535±0.077	&0.3096±0.1365	&0.010±0.004	&0.9916±0.0066&	0.500±0.001\\
        \makecell{prophet} & 160.667±14.364	&788±115.5	&19118.33±287.77&	6573.33±2952.52	&0.729±0.079	&0.171±0.021	&0.0264±0.0090	&0.96±0.006	&0.493±0.004\\
        \makecell{quadratic} & 177.33±23.71	&807±126.69	&18951±424.72	&6556.67±2953.11	&0.73±0.08	&0.18±0.01	&0.029±0.012	&0.959±0.007	&0.494±0.005 \\
        \makecell{sarima} & 97.33±3.79	&328±37.8	&19986±267.1	&6636.67±2969.4&	0.748±0.080	&0.2297±0.0141	&0.016±0.007	&0.984±0.002	&0.5±0.003 \\
        \hline
    \end{tabular}
    \end{adjustbox}

\end{comment}

==> tables/metrics.tex <==
\floatstyle{plaintop}
\restylefloat{table}
\begin{table}[H]
    %\centering
    \caption{Evaluation Metrics}
    \label{tab:evaluation_metrics}
    \begin{tabular}{p{0.45\linewidth} p{0.45\linewidth}}%{0.9\columnwidth}{XX}
        \toprule
        \textbf{Metric} & \textbf{Description} \\
        \midrule
        \multicolumn{2}{l}{\textbf{Regression}} \\
        \midrule
        MSE & Mean Squared Error \\
        \addlinespace
        RMSE & Root Mean Squared Error \\
        \addlinespace
        MAE & Mean Absolute Error \\
        \addlinespace
        \midrule
        \multicolumn{2}{l}{\textbf{Computational Complexity}} \\
        \midrule
        $t_{\text{train}}$ (s) / 1k data points & Time for training per 1k data points \\
        \addlinespace
        $t_{\text{infer}}$ (s) / 1k data points & Time for inference per 1k data points \\
        \addlinespace
        $t_{\text{train}}$ (s) / 1k nodes & Time for training per 1k nodes \\
        \addlinespace
        $t_{\text{infer}}$ (s) / 1k nodes & Time for inference per 1k nodes \\
        \addlinespace
        \midrule
        \multicolumn{2}{l}{\textbf{Alert Accuracy}} \\
        \midrule
        Avg. Daily Alerted Nodes & Average
        number of nodes alerted per day\\
        \addlinespace
        Avg. Daily Alerts & Average number of alerts per day\\
        \addlinespace
        Total Alerts & Total alerts in whole prediction time-span\\
        \addlinespace
        Avg. Alert Duration (min.) & Average alert duration\\
        \addlinespace
        Std. Alert Duration (min.) & Standard deviation alert duration\\
        \addlinespace
        Avg. Alerts per hour & Average alerts per hour\\
        \addlinespace
        Std. Alerts per hour & Standard deviation alerts per hour\\
        \addlinespace
        Accuracy & $\frac{TP + TN}{\text{Total}}$ \\
        \addlinespace
        Precision & $\frac{TP}{TP + FP}$ \\
        \addlinespace
        Recall & $\frac{TP}{TP + FN}$ \\
        \addlinespace
        Specificity & $\frac{TN}{TN + FP}$ \\
        \addlinespace
        Balanced Accuracy & $\frac{\text{Recall} + \text{Specificity}}{2}$ \\
        \bottomrule
    \end{tabular}
\end{table}
%\FloatBarrier
%\end{comment}
\begin{comment}
\begin{table}[h!]
    \centering
    \caption{Evaluation Metrics (Abbreviated)}
    \label{tab:evaluation_metrics}
    
    \begin{subtable}{0.8\columnwidth}
        \centering
        \caption{Regression Metrics}
        \begin{tabular}{@{}cl@{}}
            \toprule
            \textbf{Metric} & \textbf{Description} \\
            \midrule
            MSE & Mean Squared Error \\
            \addlinespace
            RMSE & Root Mean Squared Error \\
            \addlinespace
            MAE & Mean Absolute Error \\
            \bottomrule
        \end{tabular}
    \end{subtable}
    
    \vspace{0.5em}
    
    \begin{subtable}{0.8\columnwidth}
        \centering
        \caption{Computational and Alert Metrics}
        \begin{tabular}{@{}cl@{}}
            \toprule
            \textbf{Metric} & \textbf{Description} \\
            \midrule
            $t_{\text{train}}$ / 1k data pts & Training time per 1k data pts \\
            \addlinespace
            $t_{\text{infer}}$ / 1k data pts & Inference time per 1k data pts \\
            \addlinespace
            $t_{\text{train}}$ / 1k nodes & Training time per 1k nodes \\
            \addlinespace
            $t_{\text{infer}}$ / 1k nodes & Inference time per 1k nodes \\
            \addlinespace
            Daily Alerted Nodes & Nodes alerted per day \\
            \addlinespace
            Avg. Daily Alerts & Avg. alerts per day \\
            \addlinespace
            Total Alerts & Total alerts \\
            \addlinespace
            Avg. Alert Duration (min.) & Avg. alert duration \\
            \bottomrule
        \end{tabular}
    \end{subtable}
    
    \vspace{0.5em}
    
    \begin{subtable}{0.8\columnwidth}
        \centering
        \caption{Classification Metrics}
        \begin{tabular}{@{}cl@{}}
            \toprule
            \textbf{Metric} & \textbf{Description} \\
            \midrule
            Accuracy & $\frac{TP + TN}{\text{Total}}$ \\
            \addlinespace
            Precision & $\frac{TP}{TP + FP}$ \\
            \addlinespace
            Recall & $\frac{TP}{TP + FN}$ \\
            \addlinespace
            Specificity & $\frac{TN}{TN + FP}$ \\
            \addlinespace
            Balanced Accuracy & $\frac{\text{Recall} + \text{Specificity}}{2}$ \\
            \bottomrule
        \end{tabular}
    \end{subtable}
    
\end{table}
\end{comment}

\begin{figure}[h!]
    \centering
    \begin{tikzpicture}
        \matrix[
            matrix of nodes,
            nodes={text width=1.5cm, align=center},
            row sep=-\pgflinewidth,
            column sep=-\pgflinewidth,
            nodes in empty cells,
            row 1/.style={nodes={align=left}},
            column 1/.style={nodes={align=right}},
        ] (confusion) {
            & Actual Positive & Actual Negative \\
            Predicted Positive & TP & FP \\
            Predicted Negative & FN & TN \\
        };
        \draw[thick, dashed] (confusion-2-1.north west) -- (confusion-2-3.north east);
        \draw[thick, dashed] (confusion-1-2.north west) -- (confusion-3-2.south west);
    \end{tikzpicture}
    \caption{Confusion Matrix}
    \label{fig:confusion_matrix}
\end{figure}
\FloatBarrier



==> tables/period_high.tex <==

\floatstyle{plaintop}
\restylefloat{table}
\begin{table*}[t]
    \centering
    \caption{Performance metrics of a batch of nodes with high periodicity}
    \label{tab:period_high}
    
    \begin{adjustbox}{width=1.6\columnwidth, keepaspectratio}
    \begin{tabular}{c|c|c|c|c|c|c}
        \hline
        \makecell{\textbf{Model}} & \makecell{\textbf{MSE}} & \makecell{\textbf{RMSE}} & \makecell{\textbf{MAE}} & \makecell{\textbf{Avg. Daily Alerted} \\ \textbf{Nodes}} &  \makecell{\textbf{Avg. Daily} \\ \textbf{Alerts}}  \\
        \hline
        \makecell{arima} & 181.675	&8.116	&4.330	&53.3	&111.3 \\
        \makecell{dlm} & 212.795	&9.207&	5.590&	64.2&	143.5\\
        \makecell{lachesis\_v0} & \textbf{1.441}	&\textbf{1.143}	&\textbf{1.003}	&76.3&	188.5 \\
        \makecell{lachesis\_v1} & 2384.963	&48.532	&48.052&	\textbf{8.8}	&\textbf{16.3}\\
        \makecell{linear} & 176.812	&8.492&	5.182	&64.0	&151.3\\
        \makecell{phase1} &9280.777&	42.813&	19.870&	30.2&	49.5 \\
        \makecell{prophet} & 200.930	&8.954	&5.729	&59.2	&128.8\\
        \makecell{quadratic} & 217.408	&9.319	&6.372	&61.7	&136.0\\
        \makecell{sarima} & 303.269	&9.430&	5.714&	33.0&	56.8\\
        \hline
    \end{tabular}
    \end{adjustbox}

    \vspace{10pt}
    
    \begin{adjustbox}{width=1.6\columnwidth, keepaspectratio}
    \begin{tabular}{c|c|c|c|c}
        \hline
        \textbf{Model} & \makecell{\textbf{Avg. Alert} \\ \textbf{duration (min.)}} & \makecell{\textbf{Std. Alert} \\ \textbf{duration (min.)}} & \makecell{\textbf{Avg. Alerts} \\ \textbf{per hour}} & \makecell{\textbf{Std. Alerts} \\ \textbf{per hour}} \\
        \hline
        \makecell{arima} & 110.76&	100.127	&4.726&	2.708\\
        \makecell{dlm} & 108.68	&105.475&	6.021&	2.869 \\
        \makecell{lachesis\_v0} & 217.37&	311.608	&7.854	&3.491\\
        \makecell{lachesis\_v1} & 101.44	&\textbf{69.968}	&\textbf{1.468}&	\textbf{0.889}\\
        \makecell{linear} & 121.16	&123.672&	6.369	&3.020 \\
        \makecell{phase1} &\textbf{96.98}	&77.192	&2.753	&1.656 \\
        \makecell{prophet} & 109.34	&95.463&	5.496&	2.708\\
        \makecell{quadratic} & 114.34	&111.667&	5.693&	3.068 \\
        \makecell{sarima} & 103.73	&96.163&2.684&	1.635 \\
        \hline
    \end{tabular}
    \end{adjustbox}
    
    \vspace{10pt}

    \begin{adjustbox}{width=2.3\columnwidth, keepaspectratio}
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c}
        \hline
        \makecell{\textbf{Model}} & \makecell{\textbf{TP}} & \makecell{\textbf{FP}} & \makecell{\textbf{TN}} & \makecell{\textbf{FN}} & \makecell{\textbf{accuracy}} & \makecell{\textbf{precision}} & \makecell{\textbf{recall}} & \makecell{\textbf{specificity}}  & \makecell{\textbf{balanced accuracy}}\\
        \hline
        \makecell{arima} & 88	&580	&17153	&152	&0.959&	0.132	&0.367	&0.967&	0.667\\
        \makecell{dlm} & 97	&764&	16835&	\textbf{122}	&0.950	&0.113&	\textbf{0.443}&	0.957	&\textbf{0.700}\\
        \makecell{lachesis\_v0} & 69&	1062	&14341	&306&	0.913	&0.061	&0.184	&0.931&	0.558 \\
        \makecell{lachesis\_v1} & 44	&\textbf{54}	&\textbf{18198}	&284	&\textbf{0.982}&	\textbf{0.449}&	0.134	&\textbf{0.997}	&0.566\\
        \makecell{linear} & \textbf{101}&	807&	16562&	139	&0.946&	0.111&	0.421	&0.954	&0.687 \\
        \makecell{phase1} &33	&264	&17822	&538	&0.957&	0.111&	0.058	&0.985&	0.522\\
        \makecell{prophet} & 76	&697	&16955	&171	&0.952	&0.098&	0.308&	0.961&	0.634 \\
        \makecell{quadratic} & 92	&724	&16829	&147	&0.951&	0.113&	0.385	&0.959	&0.672 \\
        \makecell{sarima} & 54	&287	&17776	&268	&0.970	&0.158	&0.168	&0.984	&0.576 \\
        \hline
    \end{tabular}
    \end{adjustbox}
    
\end{table*}


==> tables/stationarity_full.tex <==

\floatstyle{plaintop}
\restylefloat{table}
\begin{table*}[t]
    \centering
    \caption{Performance metrics of a batch of nodes with full stationary}
    \label{tab:station_full}
    
    \begin{adjustbox}{width=1.6\columnwidth, keepaspectratio}
    \begin{tabular}{c|c|c|c|c|c|c}
        \hline
        \makecell{\textbf{Model}} & \makecell{\textbf{MSE}} & \makecell{\textbf{RMSE}} & \makecell{\textbf{MAE}} & \makecell{\textbf{Avg. Daily Alerted} \\ \textbf{Nodes}} &  \makecell{\textbf{Avg. Daily} \\ \textbf{Alerts}}  \\
        \hline
        \makecell{arima} & 3103.485	&28.589	&20.025	&38.667	&86.167\\
        \makecell{dlm} & 4180.125	&31.871	&23.351&	47.333&	111.167\\
        \makecell{lachesis\_v0} & \textbf{8.148}&	\textbf{1.857}	&\textbf{1.339}&	54.167&	142.667 \\
        \makecell{lachesis\_v1} & 2630.949	&49.714	&47.448	&\textbf{19.833}	&50.833 \\
        \makecell{linear} & 3074.893	&29.547	&22.516	&47	&120.333\\
        \makecell{phase1} &13406608.127&	1003.923&	789.627	&22.667&	\textbf{36.500}\\
        \makecell{prophet} & 5826.676	&35.251	&26.949&	45&	101.500 \\
        \makecell{quadratic} & 3484.138	&30.256	&23.721	&45.667&	105.667 \\
        \makecell{sarima} & 6604.831	&38.787	&29.096	&25.333	&45 \\
        \hline
    \end{tabular}
    \end{adjustbox}

    \vspace{10pt}
    
    \begin{adjustbox}{width=1.55\columnwidth, keepaspectratio}
    \begin{tabular}{c|c|c|c|c}
        \hline
        \textbf{Model} & \makecell{\textbf{Avg. Alert} \\ \textbf{duration (min.)}} & \makecell{\textbf{Std. Alert} \\ \textbf{duration (min.)}} & \makecell{\textbf{Avg. Alerts} \\ \textbf{per hour}} & \makecell{\textbf{Std. Alerts} \\ \textbf{per hour}} \\
        \hline
        \makecell{arima} & \textbf{102.180}	&\textbf{83.891}	&3.743&	1.874 \\
        \makecell{dlm} & 105.361	&100.870	&4.663&	2.320 \\
        \makecell{lachesis\_v0} & 307.934	&437.898&	5.975&	3.029 \\
        \makecell{lachesis\_v1} &144.803&	174.928&	2.584&	1.420 \\
        \makecell{linear} & 120.445	&118.650&	5.159&	2.447\\
        \makecell{phase1} &109.924&	94.509&\textbf{	2.229}	&\textbf{1.316}\\
        \makecell{prophet} & 110.972&	103.088&	4.374&	2.071 \\
        \makecell{quadratic} & 110.347&	106.205&	4.584&	2.192\\
        \makecell{sarima} & 113.333	&104.820&	2.390	&1.348 \\
        \hline
    \end{tabular}
    \end{adjustbox}
    
    \vspace{10pt}

    \begin{adjustbox}{width=2.3\columnwidth, keepaspectratio}
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c}
        \hline
        \makecell{\textbf{Model}} & \makecell{\textbf{TP}} & \makecell{\textbf{FP}} & \makecell{\textbf{TN}} & \makecell{\textbf{FN}} & \makecell{\textbf{accuracy}} & \makecell{\textbf{precision}} & \makecell{\textbf{recall}} & \makecell{\textbf{specificity}}  & \makecell{\textbf{balanced accuracy}}\\
        \hline
        \makecell{arima} & 117	&400	&17243	&1530&	0.900&	0.226&	0.071	&0.977	&0.524 \\
        \makecell{dlm} & 136	&531	&16970&	1401	&0.899&	0.204&	0.088	&0.970	&0.529 \\
        \makecell{lachesis\_v0} & 114	&742	&13879	&1245	&0.876	&0.133&	0.084&	0.949&	0.517 \\
        \makecell{lachesis\_v1} &126	&179	&17396	&1101&	\textbf{0.932}&\textbf{0.413}&	0.103	&0.990	&0.546\\
        \makecell{linear} & \textbf{150} &572	&16713	&\textbf{925} & 0.918	&0.208&	\textbf{0.140}	&0.967	&\textbf{0.553}\\
        \makecell{phase1} &46	&\textbf{173}	&\textbf{17616}	&2604	&0.864	&0.210&	0.017&	\textbf{0.990}&	0.504 \\
        \makecell{prophet} & 108	&501&	16983	&1919	&0.876&	0.177&	0.053&	0.971&	0.512 \\
        \makecell{quadratic} & 138	&496	&16983&	1192	&0.910	&0.218	&0.104&	0.972&	0.538 \\
        \makecell{sarima} & 72	&198	&17576&	2179&	0.881	&0.267&	0.032&	0.989&	0.510 \\
        \hline
    \end{tabular}
    \end{adjustbox}
    
\end{table*}


==> tables/tables_template.tex <==
\floatstyle{plaintop}
\restylefloat{table}
\begin{table*}[t]
    \centering
    \caption{Performance metrics of various models (filled with 0 values).}
    \label{tab:models_performance}
    
    \begin{adjustbox}{width=1.8\columnwidth, keepaspectratio}
    \begin{tabular}{c|c|c|c|c|c|c}
        \hline
        \makecell{\textbf{Model}} & \makecell{\textbf{MSE}} & \makecell{\textbf{RMSE}} & \makecell{\textbf{MAE}} & \makecell{\textbf{Daily Alerted} \\ \textbf{Nodes}} &  \makecell{\textbf{Avg. Daily} \\ \textbf{Alerts}} & \makecell{\textbf{Total Alerts}}  \\
        \hline
        \makecell{arima} & 0 & 0 & 0 & 0 & 0 & 0 \\
        \makecell{dlm} & 0 & 0 & 0 & 0 & 0 & 0 \\
        \makecell{lachesis\_v0} & 0 & 0 & 0 & 0 & 0 & 0 \\
        \makecell{lachesis\_v1} & 0 & 0 & 0 & 0 & 0 & 0 \\
        \makecell{linear} & 0 & 0 & 0 & 0 & 0 & 0 \\
        \makecell{phase1} &0 & 0& 0 & 0	& 0	& 0 \\
        \makecell{prophet} & 0 & 0 & 0 & 0 & 0 & 0 \\
        \makecell{quadratic} & 0 & 0 & 0 & 0 & 0 & 0 \\
        \makecell{sarima} & 0 & 0 & 0 & 0 & 0 & 0 \\
        \hline
    \end{tabular}
    \end{adjustbox}

    \vspace{10pt}
    
    \begin{adjustbox}{width=1.8\columnwidth, keepaspectratio}
    \begin{tabular}{c|c|c|c|c}
        \hline
        \textbf{Model} & \makecell{\textbf{t\_train (s) / 1k} \\ \textbf{data points}} & \makecell{\textbf{t\_infer (s) / 1k} \\ \textbf{data points}} & \makecell{\textbf{t\_train (s) / 1k} \\ \textbf{nodes}} & \makecell{\textbf{t\_infer (s) / 1k} \\ \textbf{nodes}} \\
        \hline
        \makecell{arima} & 0 & 0 & 0 & 0 \\
        \makecell{dlm} & 0 & 0 & 0 & 0 \\
        \makecell{lachesis\_v0} & 0 & 0 & 0 & 0 \\
        \makecell{lachesis\_v1} & 0 & 0 & 0 & 0 \\
        \makecell{linear} & 0 & 0 & 0 & 0 \\
        \makecell{phase1} &0 & 0& 0 & 0	& 0	& 0 \\
        \makecell{prophet} & 0 & 0 & 0 & 0 \\
        \makecell{quadratic} & 0 & 0 & 0 & 0 \\
        \makecell{sarima} & 0 & 0 & 0 & 0 \\
        \hline
    \end{tabular}
    \end{adjustbox}
    
    \vspace{10pt}

    \begin{adjustbox}{width=1.7\columnwidth, keepaspectratio}
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c}
        \hline
        \makecell{\textbf{Model}} & \makecell{\textbf{TP}} & \makecell{\textbf{FP}} & \makecell{\textbf{TN}} & \makecell{\textbf{FN}} & \makecell{\textbf{accuracy}} & \makecell{\textbf{precision}} & \makecell{\textbf{recall}} & \makecell{\textbf{specificity}}  & \makecell{\textbf{balanced accuracy}}\\
        \hline
        \makecell{arima} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
        \makecell{dlm} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
        \makecell{lachesis\_v0} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
        \makecell{lachesis\_v1} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
        \makecell{linear} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
        \makecell{phase1} &0 & 0& 0 & 0	& 0	& 0 \\
        \makecell{prophet} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
        \makecell{quadratic} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
        \makecell{sarima} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
        \hline
    \end{tabular}
    \end{adjustbox}
    
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%

\floatstyle{plaintop}
\restylefloat{table}
\begin{table*}[t]
    \centering
    \caption{Performance metrics of various models (filled with 0 values).}
    \label{tab:models_performance}
    
    \begin{adjustbox}{width=1.5\columnwidth, keepaspectratio}
    \begin{tabular}{c|c|c|c|c|c|c}
        \hline
        \makecell{\textbf{Model}} & \makecell{\textbf{MSE}} & \makecell{\textbf{RMSE}} & \makecell{\textbf{MAE}} & \makecell{\textbf{Total Alerted} \\ \textbf{Nodes}} &  \makecell{\textbf{Daily} \\ \textbf{Alerts}}  \\
        \hline
        \makecell{arima} & 0 & 0 & 0 & 0 & 0 & 0 \\
        \makecell{dlm} & 0 & 0 & 0 & 0 & 0 & 0 \\
        \makecell{lachesis\_v0} & 0 & 0 & 0 & 0 & 0 & 0 \\
        \makecell{lachesis\_v1} & 0 & 0 & 0 & 0 & 0 & 0 \\
        \makecell{linear} & 0 & 0 & 0 & 0 & 0 & 0 \\
        \makecell{phase1} &0 & 0& 0 & 0	& 0	& 0 \\
        \makecell{prophet} & 0 & 0 & 0 & 0 & 0 & 0 \\
        \makecell{quadratic} & 0 & 0 & 0 & 0 & 0 & 0 \\
        \makecell{sarima} & 0 & 0 & 0 & 0 & 0 & 0 \\
        \hline
    \end{tabular}
    \end{adjustbox}

    \vspace{10pt}
    
    \begin{adjustbox}{width=1.5\columnwidth, keepaspectratio}
    \begin{tabular}{c|c|c|c|c}
        \hline
        \textbf{Model} & \makecell{\textbf{Avg. Alert} \\ \textbf{duration}} & \makecell{\textbf{Std. Alert} \\ \textbf{duration}} & \makecell{\textbf{Avg. Alert} \\ \textbf{per hour}} & \makecell{\textbf{Std. Alert} \\ \textbf{per hour}} \\
        \hline
        \makecell{arima} & 0 & 0 & 0 & 0 \\
        \makecell{dlm} & 0 & 0 & 0 & 0 \\
        \makecell{lachesis\_v0} & 0 & 0 & 0 & 0 \\
        \makecell{lachesis\_v1} & 0 & 0 & 0 & 0 \\
        \makecell{linear} & 0 & 0 & 0 & 0 \\
        \makecell{phase1} &0 & 0& 0 & 0	& 0	& 0 \\
        \makecell{prophet} & 0 & 0 & 0 & 0 \\
        \makecell{quadratic} & 0 & 0 & 0 & 0 \\
        \makecell{sarima} & 0 & 0 & 0 & 0 \\
        \hline
    \end{tabular}
    \end{adjustbox}
    
    \vspace{10pt}

    \begin{adjustbox}{width=2.3\columnwidth, keepaspectratio}
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c}
        \hline
        \makecell{\textbf{Model}} & \makecell{\textbf{TP}} & \makecell{\textbf{FP}} & \makecell{\textbf{TN}} & \makecell{\textbf{FN}} & \makecell{\textbf{accuracy}} & \makecell{\textbf{precision}} & \makecell{\textbf{recall}} & \makecell{\textbf{specificity}}  & \makecell{\textbf{balanced accuracy}}\\
        \hline
        \makecell{arima} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
        \makecell{dlm} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
        \makecell{lachesis\_v0} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
        \makecell{lachesis\_v1} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
        \makecell{linear} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
        \makecell{phase1} &0 & 0& 0 & 0	& 0	& 0 \\
        \makecell{prophet} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
        \makecell{quadratic} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
        \makecell{sarima} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
        \hline
    \end{tabular}
    \end{adjustbox}
    
\end{table*}




==> tables/volatility_high.tex <==
\floatstyle{plaintop}
\restylefloat{table}
\begin{table*}[t]
    \centering
    \caption{Performance metrics of a batch of nodes with high volatility}
    \label{tab:volatility_high}
    
    \begin{adjustbox}{width=1.6\columnwidth, keepaspectratio}
    \begin{tabular}{c|c|c|c|c|c|c}
        \hline
        \makecell{\textbf{Model}} & \makecell{\textbf{MSE}} & \makecell{\textbf{RMSE}} & \makecell{\textbf{MAE}} & \makecell{\textbf{Avg. Daily Alerted} \\ \textbf{Nodes}} &  \makecell{\textbf{Avg. Daily} \\ \textbf{Alerts}}  \\
        \hline
        \makecell{arima} & 8574.378	&56.854	&44.696	&12.5	&27.5 \\
        \makecell{dlm} & 12175.386	&65.003	&50.037&	14.5	&31.5 \\
        \makecell{lachesis\_v0} & \textbf{21.970}	&\textbf{3.050}	&\textbf{2.027}	&16.833&	41.333 \\
        \makecell{lachesis\_v1} & 3429.130	&54	&46.379	&9.667	&25.833\\
        \makecell{linear} & 8657.113	&60.636	&51.350	&13.667	&32 \\
        \makecell{phase1} &45179583.240	&3128.713	&2521.655	&7.167	&12.167 \\
        \makecell{prophet} & 17761.725	&76.574	&61.494&	15.167&	31.500\\
        \makecell{quadratic} & 9752.012	&58.776	&49.066	&14.5	&32 \\
        \makecell{sarima} & 19906.523	&86.075	&68.089&	\textbf{6.667}	&\textbf{10.833}\\
        \hline
    \end{tabular}
    \end{adjustbox}

    \vspace{10pt}
    
    \begin{adjustbox}{width=1.55\columnwidth, keepaspectratio}
    \begin{tabular}{c|c|c|c|c}
        \hline
        \textbf{Model} & \makecell{\textbf{Avg. Alert} \\ \textbf{duration (min.)}} & \makecell{\textbf{Std. Alert} \\ \textbf{duration (min.)}} & \makecell{\textbf{Avg. Alerts} \\ \textbf{per hour}} & \makecell{\textbf{Std. Alerts} \\ \textbf{per hour}} \\
        \hline
        \makecell{arima} & 154.322	&177.520&	1.823	&0.954\\
        \makecell{dlm} & 118.017	&102.821&	1.765	&0.964 \\
        \makecell{lachesis\_v0} & 396.687	&536.435&	2.167&	1.411 \\
        \makecell{lachesis\_v1} & 172.856	&226.995&	1.720&	0.929 \\
        \makecell{linear} & 159.310	&153.114	&1.883	&1.072 \\
        \makecell{phase1} &137.501	&102.494&	1.384	&0.511 \\
        \makecell{prophet} & 139.667&	130.948	&1.759&	1.049 \\
        \makecell{quadratic} &132.414	&125.119&	1.893	&1.090 \\
        \makecell{sarima} & \textbf{107.337}	&\textbf{78.960}&	\textbf{1.232}&	\textbf{0.407}\\
        \hline
    \end{tabular}
    \end{adjustbox}
    
    \vspace{10pt}

    \begin{adjustbox}{width=2.3\columnwidth, keepaspectratio}
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c}
        \hline
        \makecell{\textbf{Model}} & \makecell{\textbf{TP}} & \makecell{\textbf{FP}} & \makecell{\textbf{TN}} & \makecell{\textbf{FN}} & \makecell{\textbf{accuracy}} & \makecell{\textbf{precision}} & \makecell{\textbf{recall}} & \makecell{\textbf{specificity}}  & \makecell{\textbf{balanced accuracy}}\\
        \hline
        \makecell{arima} &33	&132	&17880&	1331&	0.924&	0.200&	0.024	&0.993	&0.508 \\
        \makecell{dlm} & 46	&143&	17942&	1222&	0.929&	0.243&	0.036&	0.992&	0.514 \\
        \makecell{lachesis\_v0} & 56	&192&	16758&	917&	0.938&	0.226&	0.058&	0.989	&0.523\\
        \makecell{lachesis\_v1} & \textbf{59}	&96	&17905&	841	&0.950&	\textbf{0.381}&\textbf{	0.066}&	0.995&	\textbf{0.530} \\
        \makecell{linear} & 47	&145	&17807&	\textbf{765}&	\textbf{0.952}&	0.245&	0.058&	0.992&	0.525 \\
        \makecell{phase1} &21	&52	&18108	&2015	&0.898&	0.288&	0.010&	0.997&	0.504 \\
        \makecell{prophet} & 37	&152&	17864&	1701&	0.906&	0.196&	0.021&	0.992&	0.506 \\
        \makecell{quadratic} & 52	&140&	17899&	999&	0.940&	0.271	&0.049	&0.992&	0.521 \\
        \makecell{sarima} & 22	&\textbf{43}	&\textbf{18176}	&1876	&0.905	&0.338&	0.012&	\textbf{0.998}&	0.505\\
        \hline
    \end{tabular}
    \end{adjustbox}
    
\end{table*}




==> tables/week26_unbalanced_res.tex <==
\floatstyle{plaintop}
\restylefloat{table}
\begin{table*}[t]
    \centering
    \caption{Performance metrics of random batch of nodes}
    \label{tab:random_batch}
    
    \begin{adjustbox}{width=1.7\columnwidth, keepaspectratio}
    \begin{tabular}{c|c|c|c|c|c|c}
        \hline
        \makecell{\textbf{Model}} & \makecell{\textbf{MSE}} & \makecell{\textbf{RMSE}} & \makecell{\textbf{MAE}} & \makecell{\textbf{Avg. Daily Alerted} \\ \textbf{Nodes}} &  \makecell{\textbf{Avg. Daily} \\ \textbf{Alerts}} & \makecell{\textbf{Total Alerts}}  \\
        \hline
        \makecell{arima} & 716.583	&26.769	&4.562 & 160.571	&313.714	&2196 \\
        \makecell{dlm} & 597.177	& 24.437	& 3.974 & 177.571	&386.143	&2703 \\
        \makecell{lachesis\_v0} & 4949.280	&70.351	&9.078 & 163	&360.571	&2524\\
        \makecell{lachesis\_v1} & 8736.745	&93.471	&22.241 & \textbf{60}	& \textbf{102.143}	&\textbf{715}\\
        \makecell{linear} & 526.723	&22.950	&\textbf{3.885} & 180.286	&396.571	&2776 \\
        \makecell{phase1} & 856168.325	&925.294	&68.259	& 84.571&134.571	&942\\
        \makecell{prophet} & 770.622	&27.760	&4.521 &172.143	&353.143	&2472 \\
        \makecell{quadratic} &\textbf{439.302}	&\textbf{20.960}	&3.982 & 175.286	&374.429	&2621 \\
        \makecell{sarima} & 809.139	&28.445	&5.115 & 91.714	&150.714	&1055 \\
        \hline
    \end{tabular}
    \end{adjustbox}

    \vspace{10pt}
    
    \begin{adjustbox}{width=1.6\columnwidth, keepaspectratio}
    \begin{tabular}{c|c|c|c|c}
        \hline
        \textbf{Model} & \makecell{\textbf{t\_train (s) / 1k} \\ \textbf{data points}} & \makecell{\textbf{t\_infer (s) / 1k} \\ \textbf{data points}} & \makecell{\textbf{t\_train (s) / 1k} \\ \textbf{nodes}} & \makecell{\textbf{t\_infer (s) / 1k} \\ \textbf{nodes}} \\
        \hline
        \makecell{arima} & 1.361	&0.368	&1144.211&	62.170 \\
        \makecell{dlm} &0.950	&1.971	&798.570	&333.054\\
        \makecell{lachesis\_v0} & 0.142	&34.909	&7177.615	&5899.608\\
        \makecell{lachesis\_v1} & 0.235 & \textbf{0.001} & 11853.574&\textbf{0.169}\\
        \makecell{linear} & 0.008&	0.043	&6.741	&7.257\\
        \makecell{phase1} &\textbf{0.0016}&	0.029	&\textbf{1.359}	&4.886\\
        \makecell{prophet} & 0.261	&0.780	&219.092	&131.865\\
        \makecell{quadratic} & 0.010	&0.044	&8.368&	7.461 \\
        \makecell{sarima} & 4.892	&0.355	&4114.328	&59.971 \\
        \hline
    \end{tabular}
    \end{adjustbox}
    
    \vspace{10pt}

    \begin{adjustbox}{width=2\columnwidth, keepaspectratio}
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c}
        \hline
        \makecell{\textbf{Model}} & \makecell{\textbf{TP}} & \makecell{\textbf{FP}} & \makecell{\textbf{TN}} & \makecell{\textbf{FN}} & \makecell{\textbf{accuracy}} & \makecell{\textbf{precision}} & \makecell{\textbf{recall}} & \makecell{\textbf{specificity}}  & \makecell{\textbf{balanced accuracy}}\\
        \hline
        \makecell{arima} & 0	&2196	&48783	&0	&0.957	&0	&	&0.957&	\\
        \makecell{dlm} & 0	&2703	&48230	&0	&0.947	&0	&	&0.947&	\\
        \makecell{lachesis\_v0} & 0&	2524	&46754	&0	&0.949	&0	&	&0.949&	\\
        \makecell{lachesis\_v1} & 0	&\textbf{715}	&51313&	0	&\textbf{0.986}	&0	&	&\textbf{0.986}	& \\
        \makecell{linear} & 0	&2776	&47213	&0	&0.944	&0	&	&0.944	& \\
        \makecell{phase1} &0	&942	&\textbf{51480}	&0	&0,982	&0	&	&0,982&\\
        \makecell{prophet} & 0	&2472	&48503	&0	&0.952	&0	&	&0.952	& \\
        \makecell{quadratic} & 0	&2621	&47958	&0	&0.948	&0&	&	0.948&	\\
        \makecell{sarima} & 0	&1055	&51307	&0	&0.980	&0	&	&0.980	& \\
        \hline
    \end{tabular}
    \end{adjustbox}
    
\end{table*}



